A Multi-Party, Multi-Blockchain Atomic Swap Protocol with Universal Adaptor Secret

The increasing complexity of digital asset transactions across multiple blockchains necessitates a robust atomic swap protocol that can securely handle more than two participants. Traditional atomic swap protocols, including those based on adaptor signatures, are vulnerable to malicious dropout attacks, which break atomicity and compromise the security of the transaction. This paper presents a novel multi-party atomic swap protocol that operates almost entirely off-chain, requiring only a single on-chain transaction for finalization. Our protocol leverages Schnorr-like signature verification and a universal adaptor secret to ensure atomicity and scalability across any number of participants and blockchains without the need for smart contracts or trusted third parties. By addressing key challenges such as collusion attacks and malicious dropouts, our protocol significantly enhances the security and efficiency of multi-party atomic swaps. Our contributions include the first scalable, fully off-chain protocol for atomic swaps involving any number of participants, adding zero overhead to native blockchains, and providing a practical and cost-effective solution for decentralized asset exchanges.

==> src/comments.tex <==
%%
%% This is file `sample-sigconf.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% samples.dtx  (with options: `sigconf')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from sample-sigconf.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file samples.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%%
%% Commands for TeXCount
%TC:macro \cite [option:text,text]
%TC:macro \citep [option:text,text]
%TC:macro \citet [option:text,text]
%TC:envir table 0 1
%TC:envir table* 0 1
%TC:envir tabular [ignore] word
%TC:envir displaymath 0 word
%TC:envir math 0 word
%TC:envir comment 0 0
%%
%%

%% The first command in your LaTeX source must be the \documentclass command.

%%%%%%



==> src/commonts.tex <==
% LLNCS macro package for Springer Computer Science proceedings;
% Version 2.21 of 2022/01/12
%

%%%%%



==> src/tables/table_related_works_bridge_compare.tex <==
\begin{table*}[htbp]
    \begin{threeparttable}
        \caption{Comparison of Cross-Chain Interoperability Approaches}
        \centering
        \begin{tabular}{|p{3.5cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|}
            \hline
            \textbf{Approach} & \textbf{Double-Spending Resistance} & \textbf{Collusion Resistance} & \textbf{Transaction Privacy} & \textbf{Decentralized} & \textbf{Atomicity} \\
            \hline
            Atomic Swap & \checkmark Schulte et al. \cite{schulte2019towards} & \textcolor{red}{\ding{55}} Haugum et al. \cite{haugum2022security} & \checkmark Deshpande et al. \cite{deshpande2020privacy} & \checkmark Sigwart et al. \cite{sigwart2021decentralized} & \checkmark Zakhary et al. \cite{zakhary2019atomic} \\
            \hline
            Sidechain & \textcolor{red}{\ding{55}} Haugum et al. \cite{haugum2022security} & \textcolor{red}{\ding{55}} Haugum et al. \cite{haugum2022security} & \checkmark Parizi et al. \cite{parizi2019integrating} & \checkmark Johnson et al. \cite{johnson2019sidechains} & \checkmark Pillai et al. \cite{pillai2022cross} \\
            \hline
            Token-Wrapping & \checkmark Caldarelli et al. \cite{caldarelli2021wrapping} & \textcolor{red}{\ding{55}}\tnote{$\mp$}\hspace{2mm} Ren et al. \cite{ren2023interoperability} & \textcolor{red}{\ding{55}} Caldarelli et al. \cite{caldarelli2021wrapping} & \checkmark Dilley et al. \cite{dilley2016strong} & \checkmark Barbàra et al. \cite{9922019} \\
            \hline
            Notary and Relay Schemes & \checkmark Nicolas et al. \cite{nicolas2020blockchain} & \checkmark Haugum et al. \cite{haugum2022security} & \textcolor{red}{\ding{55}} Lan et al. \cite{lan2021trustcross} & \checkmark Sun et al. \cite{sun2022decentralized} & \checkmark Lys et al. \cite{lys2020atomic} \\
            \hline
            Our Protocol \tnote{$\dag$}\hspace{2mm} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
            \hline
        \end{tabular}
        \label{tab:compare-bridges}
        \centering
        \begin{tablenotes}\footnotesize
            \item[$\mp$] This approach does not inherently support the given characteristic.
            \item[$\dag$] Cross-blockchain data validation oracle protocol based on LLM-agents.
        \end{tablenotes}
    \end{threeparttable}
\end{table*}

==> src/tables/table_security.tex <==
\begin{table*}[htbp]
    \begin{center}
        \begin{tabular}{|p{3.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
            \hline
            \textbf{Bridge Protocol} & \textbf{Trustless} & \textbf{Collusion Resistance} & \textbf{MEV Resistance} & \textbf{Transaction Privacy} \\
            \hline
            Atomic Swap & \checkmark & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} \\
            \hline
            Sidechain and Token-Wrapping & \checkmark & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} \\
            \hline
            Notary and Relay Schemes & \checkmark & \checkmark & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} \\
            \hline
            Burn-and-Mint (Our Design) & \checkmark & \checkmark & \checkmark & \checkmark \\
            \hline
        \end{tabular}
    \end{center}
    \caption{Comparison of Bridge Protocols}
    \label{tab:security}
\end{table*}

==> src/tables/table_security_proof_notation.tex <==
\begin{table*}[ht]
    \centering
    \caption{Table of Notations}
    \resizebox{0.8 \textwidth}{!}{
    \begin{tabular}{|c|l|c|l|}
        \hline
        \textbf{Symbol} & \textbf{Definition} & \textbf{Symbol} & \textbf{Definition} \\
        \hline
        $\mathcal{P}$ & Burn-and-Mint protocol & $\mathcal{E}_p$ & Proposed exchange rate \\
        \hline
        $\mathcal{B}_1$, $\mathcal{B}_2$ & Original and destination blockchains & $\mathcal{D}_{r}$ & Dispute by relay $r$ \\
        \hline
        $\mathcal{U}$ & Set of users & $\mathcal{S}_{r}$ & Stake of relay $r$ \\
        \hline
        $\mathcal{R}$ & Set of relays & $\mathcal{F}_{r}$ & Forfeit of stake \\
        \hline
        $\mathcal{T}$ & Timestamp function & $\mathcal{A}$ & The adversary \\
        \hline
        $\mathcal{K}$ & Key generation algorithm & $\mathcal{I}$ & Information function \\
        \hline
        $\mathcal{Z}$ & ZKP scheme & $\varepsilon$ & Negligible quantity \\
        \hline
        $\text{PrK}_{u}$ & Private key of user $u$ & $\mathcal{M}_{\mathcal{A}}$ & Adversary's query set \\
        \hline
        $\text{PuK}_{u}$ & Public key of user $u$ & $\sigma$ & Valid message-signature pair \\
        \hline
        $\tau$ & Token swap transaction & $\mathcal{N}_{u}$ & Unique nullifier \\
        \hline
        $\tau_{b}$ & Burn transaction & $C_{u}$ & User's commitment \\
        \hline
        $\tau_{m}$ & Mint transaction & $\mathcal{E}$ & Exchange rate \\
        \hline
        $\pi_{u}$ & ZKP of token ownership & $\text{Pr}[\cdot]$ & Probability Function \\
        \hline
    \end{tabular}
    }
    \label{tab:notation}
\end{table*}

